Branching exponents of synthetic vascular trees under different optimality principles

The branching behavior of vascular trees is often characterized using Murray's law. We investigate its validity using synthetic vascular trees generated under global optimization criteria. Our synthetic tree model does not incorporate Murray's law explicitly. Instead, we assume it holds implicitly and investigate the effects of different physical constraints and optimization goals on the branching exponent that is now allowed to vary locally. In particular, we include variable blood viscosity due to the F{\aa}hr{\ae}us--Lindqvist effect and enforce an equal pressure drop between inflow and the micro-circulation. Using our global optimization framework, we generate vascular trees with over one million terminal vessels and compare them against a detailed corrosion cast of the portal venous tree of a human liver. Murray's law is implicitly fulfilled when no additional constraints are enforced, indicating its validity in this setting. Variable blood viscosity or equal pressure drop leads to deviations from this optimum, but with the branching exponent inside the experimentally predicted range between 2.0 and 3.0. The validation against the corrosion cast shows good agreement from the portal vein down to the venules. Not enforcing Murray's law explicitly reduces the computational cost and increases the predictive capabilities of synthetic vascular trees. The ability to study optimal branching exponents across different scales can improve the functional assessment of organs.

==> aomacros.tex <==
\usepackage{booktabs}
\usepackage{siunitx}
\usepackage{xspace}
\usepackage{cite}

\usepackage{./input/luh-colors}
\usepackage{./input/ao-math-std}
\usepackage{./input/ao-math-graphs}
\usepackage{./input/ao-math-fields}

\newcommand\mcs[2][]{\textcolor{LUH-red}{#2}\drop{#1}\xspace}
\newcommand\new[2][]{\textcolor{LUH-blue}{#2}\drop{#1}\xspace}
\newcommand\drop{\textcolor{LUH-green}}
\newcommand\orcauth[2]{\href{https://orcid.org/#1}
  {\includegraphics[height=0.7em]{template/orcid.pdf}\enspace#2}}
\newcommand\con{\tsb{con}}
\newcommand\geo{\tsb{geo}}
\newcommand\perf{\tsb{perf}}
\newcommand\term{\tsb{term}}
\newcommand\CCO{\tsp{in}}
\colorlet{imgcol}{LUH-green}
\newcommand\image[2][]{\bgroup\fboxsep0pt\fboxrule0.2pt
  \protect\fcolorbox{imgcol}{imgcol!10}{\protect\includegraphics[#1]{#2}}\egroup}


==> input/math-fields.tex <==
% Math fields -- requires amsfonts

\newcommand{\field}{\mathbb}

% "natural" names
\newcommand{\complex}{\field{C}}
\newcommand{\quaternions}{\field{H}}
\newcommand{\naturals}{\field{N}}
\newcommand{\polynomials}{\field{P}}
\newcommand{\rationals}{\field{Q}}
\newcommand{\reals}{\field{R}}
\newcommand{\integers}{\field{Z}}

% alternative names
\newcommand{\numsetC}{\complex}
\newcommand{\numsetH}{\quaternions}
\newcommand{\numsetN}{\naturals}
\newcommand{\numsetQ}{\rationals}
\newcommand{\numsetR}{\reals}
\newcommand{\numsetZ}{\integers}

% short names
\makeatletter
\@ifundefined{C}{\newcommand{\C}{\complex}}
{\PackageInfo{math-fields}{Use \string\field{C} for complex numbers;
 \MessageBreak command \string\C\space already defined}{}}
\makeatother
\newcommand{\N}{\naturals}
\newcommand{\Q}{\rationals}
\newcommand{\R}{\reals}
\newcommand{\Z}{\integers}
\newcommand{\Poly}{\polynomials}% deprecated: NuMa scripts


==> input/math-graphs.tex <==
% Graph macros -- requires amsfonts and math-symbols

% Set of graph elements.
\newcommand{\graphset}{\mathbb}
\newcommand{\graphindex}{\tsb}% alternative: \tsp

\newcommand{\Graph}{\graphset{G}}
\newcommand{\Arcs}{\ensuremath{\graphset{A}}}
\newcommand{\Edges}{\graphset{E}}
\newcommand{\Nodes}{\graphset{V}}
\newcommand{\Vertices}{\Nodes}

\newcommand\Tree{\graphset{T}}
\newcommand\Level{\graphset{L}}
\newcommand\Leaves{\graphset{L}}

\newcommand{\node}{i}
\newcommand{\otherNode}{j}
\newcommand{\vertex}{v}
\newcommand{\otherVertex}{u}
\newcommand{\edge}{e}
\newcommand{\arc}{a}

\newcommand{\Arc}[1]{\Arcs\graphindex{#1}}
\newcommand{\Edge}[1]{\Edges\graphindex{#1}}
\newcommand{\Node}[1]{\Nodes\graphindex{#1}}
\newcommand{\Vertex}[1]{\Vertices\graphindex{#1}}

\newcommand{\BufNodes}{\Node{buf}}
\newcommand{\CtrlArcs}{\Arc{ctrl}}

\newcommand{\Junctions}{\Nodes_0}
\newcommand{\Sources}{\Nodes_+}
\newcommand{\Entries}{\Sources}
\newcommand{\Sinks}{\Nodes_-}
\newcommand{\Exits}{\Sinks}
\newcommand{\Heads}{\delta^+}
\newcommand{\Tails}{\delta^-}
\newcommand{\BoundaryNodes}{{\Nodes^\circ}}


\newcommand{\cardA}{\card{\Arcs}}
\newcommand{\cardE}{\card{\Edges}}
\newcommand{\cardN}{\card{\Nodes}}
\newcommand{\cardV}{\card{\Vertices}}

\newcommand{\IncMat}{E}% incidence matrix


==> input/math-std.tex <==
% Standard math definitions -- requires amsmath

\newcommand\const{\textup{const}}
\newcommand\qtext{\quad\text}
\newcommand\textq[1]{\text{#1}\quad}
\newcommand\qtextq{\quad\textq}
\newcommand\st{\textup{s.t.}}
\newcommand\stq{\st\quad}
\newcommand\qst{\quad\st}
\newcommand\qstq{\qst\quad}

\makeatletter
\newcommand\fcdot{\,\cdot\,}
\newcommand\ifgiven[3]{\def\fc@rg{#1}\ifx\fc@rg\empty#3\else#2\fi}
\newcommand\fcarg[1]{\ifgiven{#1}\fc@rg\fcdot}
\makeatother
\newcommand\abs[1]{\lvert\fcarg{#1}\rvert}
\newcommand\Abs[1]{\left\lvert#1\right\rvert}
\newcommand\tfracabs[2]{\abs{#1}/\abs{#2}}
\newcommand\fracabs[2]{\frac{\abs{#1}}{\abs{#2}}}
\newcommand\fracAbs[2]{\frac{\Abs{#1}}{\Abs{#2}}}
\newcommand\tabsfrac\tfracabs
\newcommand\absfrac\fracabs
\newcommand\Absfrac\fracAbs
\newcommand\card\abs
\newcommand\Card\Abs
\newcommand\ceil[1]{\lceil\fcarg{#1}\rceil}
\newcommand\Ceil[1]{\left\lceil#1\right\rceil}
\newcommand\defsep\colon% alternative: \mid
\newcommand\defset[3][\defsep]{\set{#2#1#3}}
\newcommand\Defset[3][\defsep]{\Set{#2#1#3}}
\newcommand\EEmult\cdot% alternative: \times
\newcommand\EE[1][\EEmult]{#1 10^}
\newcommand\floor[1]{\lfloor\fcarg{#1}\rfloor}
\newcommand\Floor[1]{\left\lfloor#1\right\rfloor}
\newcommand\Inv[1]{#1^{-1}}
\newcommand\HInv[1]{#1\ihr}% hermitian inverse
\newcommand\TInv[1]{#1\itp}% transpose inverse
\newcommand\norm[2][]{\lVert\fcarg{#2}\rVert\optsb{#1}}
\newcommand\Norm[2][]{\left\lVert#2\right\rVert\optsb{#1}}
\newcommand\tfracnorm[3][]{\norm[#1]{#2}/\norm[#1]{#3}}
\newcommand\fracnorm[3][]{\frac{\norm[#1]{#2}}{\norm[#1]{#3}}}
\newcommand\fracNorm[3][]{\frac{\Norm[#1]{#2}}{\Norm[#1]{#3}}}
\newcommand\tnormfrac\tfracnorm
\newcommand\normfrac\fracnorm
\newcommand\Normfrac\fracNorm
\newcommand\tfracnormpow[4][]{\norm[#1]{#2}^{#4}/\norm[#1]{#3}^{#4}}
\newcommand\fracnormpow[4][]{\frac{\norm[#1]{#2}^{#4}}{\norm[#1]{#3}^{#4}}}
\newcommand\fracNormpow[4][]{\frac{\Norm[#1]{#2}^{#4}}{\Norm[#1]{#3}^{#4}}}
\newcommand\pfrac[2]{\frac{\partial#1}{\partial#2}}
\newcommand\ppfrac[3]{\pfrac{^2#1}{#2\partial#3}}
\newcommand\set[1]{\{#1\}}
\newcommand\Set[1]{\left\{#1\right\}}
\newcommand\snorm[2][]{\lvert\!\lvert\!\lvert
  \fcarg{#2}\rvert\!\rvert\!\rvert\optsb{#1}}
\newcommand\Snorm[2][]{\left\lvert\!\left\lvert\!\left\lvert
  #2\right\rvert\!\right\rvert\!\right\rvert\optsb{#1}}
\newcommand\sprod[3][]{\langle\fcarg{#2},\fcarg{#3}\rangle\optsb{#1}}
\newcommand\Sprod[3][]{\left\langle#2,#3\right\rangle\optsb{#1}}

\newcommand\hrchar{H}
\newcommand\tpchar{T}
\newcommand\hr{^\hrchar}% hermitian transpose
\newcommand\tp{^\tpchar}
\newcommand\ihr{^{-\hrchar}}
\newcommand\itp{^{-\tpchar}}
\newcommand\tadj[1]{\mskip#1\thinmuskip}% adjust space
\newcommand\hra[1][0]{^{\tadj{#1}\hrchar}}
\newcommand\tpa[1][0]{^{\tadj{#1}\tpchar}}
\newcommand\ihra[1][0]{^{\tadj{#1}{-}\hrchar}}
\newcommand\itpa[1][0]{^{\tadj{#1}{-}\tpchar}}
\newcommand\tpfrac[2]{\tfrac{\partial#1}{\partial#2}}
\newcommand\tppfrac[3]{\tpfrac{^2#1}{#2\partial#3}}
\newcommand\without{\setminus\set}
\newcommand\Without{\setminus\Set}

\newcommand\lbound{-}
\newcommand\ubound{+}
\newcommand\splb{^{\lbound}}
\newcommand\spub{^{\ubound}}
\newcommand\sblb{_{\lbound}}
\newcommand\sbub{_{\ubound}}
\newcommand\bounds[1]{\ensuremath{[#1\splb,#1\spub]}}
\newcommand\Bounds[1]{\ensuremath{\left[#1\splb,#1\spub\right]}}

\newcommand\Strut{\rule[2.5555ex]{0pt}{0pt}}% ~1.1em
\newcommand\Hline{\hline\Strut}

\newcommand\optsb[1]{\ifgiven{#1}{_{#1}}{}}
\newcommand\optsp[1]{\ifgiven{#1}{^{#1}}{}}
\newcommand\optindex[1]{\ifgiven{#1}{,#1}{}}
\newcommand\optmathsb\optsb
\newcommand\optmathsp\optsp
\newcommand\opttextsb[1]{\optsb{\textup{#1}}}
\newcommand\opttextsp[1]{\optsp{\textup{#1}}}
\newcommand\optmathindex\optindex
\newcommand\opttextindex[1]{\optindex{\textup{#1}}}

\newcommand\define{\mathrel{{\mathop:}{=}}}
\newcommand\enifed{\mathrel{{=}{\mathop:}}}


==> input/math-symbols.tex <==
% Math symbols -- requires amsmath

% Redefine some macros in math mode. Keep text mode definitions.
\let\TeXbar\_   % underscore -> \bar
\let\TeXhat\^   % undefined  -> \hat
\let\TeXtilde\~ % undefined  -> \tilde
\let\TeXcolon\: % \tmspace+\medmuskip{.2222em} -> \colon
\makeatletter
\newcommand\mcs@cc[3]{\leavevmode\ifmmode#1{#3}\else#2{#3}\fi}
\renewcommand\_{\mcs@cc\bar\TeXbar}
\renewcommand\^{\mcs@cc\hat\TeXhat}
\renewcommand\~{\mcs@cc\tilde\TeXtilde}
\renewcommand\:{\mcs@cc\colon\TeXcolon\relax}
\makeatother
\PackageInfo{math-symbols}{Redefining
 \string\_, \string\^, \string\~, \string\: in math mode.
 \MessageBreak Keeping text mode definitions.
 \MessageBreak Saving original commands as \string\TeXbar, \string\TeXhat,
 \MessageBreak \string\TeXtilde, \string\TeXcolon}

\newcommand\0\emptyset
\newcommand\bigM{M}
\newcommand\bigO{O}
\newcommand\smallo{o}
\newcommand\oo\infty
\newcommand\ox\otimes
\newcommand\x\times

\newcommand\itxt{\textup}% text in math indices
\newcommand\tsb[1]{_{\itxt{#1}}}% text subindex
\newcommand\tsp[1]{^{\itxt{#1}}}% text superindex

\newcommand\boundary\partial
\newcommand\cond\kappa
\newcommand\condabs{\cond\tsb{abs}}\newcommand\abscond\condabs
\newcommand\condrel{\cond\tsb{rel}}\newcommand\relcond\condrel
\newcommand\convrad\rho
\newcommand\eps\epsilon
\newcommand\veps\varepsilon
\newcommand\epsM{\veps\tsb{M}}
\let\epsmach\epsM
\newcommand\specrad\rho
\newcommand\spectrum\sigma
\newcommand\uvec{\mathbf1}

% Some arrows.
\newcommand\larrow\leftarrow
\newcommand\rarrow\to% \rightarrow
\newcommand\swap\leftrightarrow
\newcommand\lrarrow\swap
\newcommand\Larrow\longleftarrow
\newcommand\Rarrow\longrightarrow
\newcommand\LRarrow\longleftrightarrow
\newcommand\xlarrow\xleftarrow
\newcommand\xrarrow\xrightarrow
\newcommand\lArrow\Leftarrow
\newcommand\rArrow\Rightarrow

% Right-shifted relation symbols for alignment with :=
\newcommand\crel[1]{\mathrel{\hphantom:{#1}}}
\newcommand\isom{\crel\cong}
\newcommand\eqls{\crel=}


==> mypackages.tex <==
\usepackage{./template/arxiv}

\usepackage{algorithm} 
\usepackage{algpseudocode} 
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage[english]{babel}
\usepackage{caption}
\usepackage{doi}
\usepackage{enumitem}
\usepackage{float}
\usepackage{graphicx}
\usepackage{hyperref} 
\usepackage[capitalise]{cleveref}
\usepackage{mathptmx}
\usepackage{microtype}
%\usepackage{natbib}
\usepackage{subfig}
\usepackage{tabularx}
\usepackage[utf8]{inputenc}


\newcommand{\mc}[3]{\multicolumn{#1}{#2}{#3}}
